Good edge-labelings and graphs with girth at least five

A good edge-labeling of a graph [Ara\'ujo, Cohen, Giroire, Havet, Discrete Appl. Math., forthcoming] is an assignment of numbers to the edges such that for no pair of vertices, there exist two non-decreasing paths. In this paper, we study edge-labeling on graphs with girth at least 5. In particular we verify, under this additional hypothesis, a conjecture by Ara\'ujo et al. This conjecture states that if the average degree of G is less than 3 and G is minimal without an edge-labeling, then G \in {C_3,K_{2,3}}. (For the case when the girth is 4, we give a counterexample.)

==> babaks-noWindmill-pf.tex <==

















\dotfill


Let~$G$ be as in the theorem.
%%
We fix a windmill~$W$ in~$G$, denote its axis by~$y$, and let $H$ be the subgraph of~$G$ induced by the windmill and its flags.

\begin{lemma}
  If $W$ contains no evil wheels, then there is
  \begin{itemize}
  \item a set of types $\tau$ for which every flag is a type-2 vertex while $\tau(y) \le 1$, and
  \item a decent edge-labeling $\phi$,
  \end{itemize}
  such that $(H,\tau,\phi, y)$ is gluable.
\end{lemma}

\begin{proof}
  We consider the list of such forbidden windmills by going over their representation in the form of a flag graph.  First, we consider the possibilities for a strong
  connected component in the flag graph.  A strongly connected component~$S$ can be either a single sail vertex or an even cycle.  (As we explained earlier, such a
  cycle can be of length~2 when we have anti-parallel edges.)
  %%
  We show that unless such a cycle represents an evil wheel, $H$ is decent.

  We do this by induction on the number of strong connected components of the flag graph.  Note that in the inductive argument, the axis is always type-0 or type-1.

  % A single vertex (only axis)

  Case~I: The flag graph is empty; that is, $H$ contains a single vertex~$y$ (i.e., the axis) and no sail.  Let~$\tau$ assign to~$y$ either type-0 or type-1, and
  let~$\phi$ be an ``empty'' edge-labeling.  Since $H$ has no edge and only one type-0 or type-1 vertex, it can be easily seen that all conditions of
  Definition~\ref{def24} are valid, and so $(H,\tau,\phi, y)$ is gluable.


  Induction step

  Case II: The flag forest has an isolated vertex.  This isolated vertex represent a strongly connected component in the flag graph which can only be a single sail
  vertex or an even cycle of length at least two.

  First assume that it is a sail vertex.  Then the sail vertex represents in $H$ either one sail or two sails sharing the same 2-vertex.  We have the following two
  subcases.

  % Attaching a sail to axis
  Case II.(a): $H$ is formed by a windmill $H_1$ with axis $y_1$ and a sail $H_2$ that ends in $y_2$ where $y_1$ and $y_2$ are identified.  By induction, there are
  types~$\tau_1$ in which~$y_1$ is not of type-2, and a decent edge-labeling $\phi_1$ such that $(H_1,\tau_1,\phi_1, y_1)$ is gluable.  Now, $H_2$ matches
  Example~\ref{exp:gluing:fishAndCycle}, the top picture in Fig.~\ref{fig:gluing:fishAndCycle}: $xv_1$ is the tip of the sail, $w$ is the other neighbour of the
  2-vertex $x$, and $v_n$ is the axis, i.e. , $y_2$.  So, there is a set of types $\tau_2$ in which $y_2$ is not a 2-type and a decent edge-labeling $\phi_2$ where
  $(H_2,\tau_2,\phi_2, y_2)$ is gluable.  Now graph $H$ is obtained from the glueing of $H_1$ and $H_2$ along $\{y_1=y_2\}$ (denote the identified vertex $y$) in
  which $y$ is type-0 or type-1.  By Lemma~\ref{lem:glue:edge}, $(H,\tau,\phi, y)$ is gluable where $\tau$ and $\phi$ are set as explained in the Lemma.


  % Attaching a degenerate sail to axis
  Case II.(b): $H$ is formed by a windmill $H_1$ with axis $y_1$ and graph $H_2$ that consists of two sails sharing the same 2-vertex and the same end $y_2$ where
  $y_1$ and $y_2$ are identified.  By induction, there is a set of types $\tau_1$ in which $y_1$ is not a type-2 and a decent edge-labeling $\phi_1$ where
  $(H_1,\tau_1,\phi_1, y_1)$ is gluable.  Now, consider Example~\ref{18} that represents $H_2$ as follows: $u$ is the 2-vertex shared by both sails, $y$ is the end
  the two sail, i.e. , $y_2$.  So, there is a set of types $\tau_2$ in which $y_2$ is not a 2-type and a decent edge-labeling $\phi_2$ where $(H_2,\tau_2,\phi_2,
  y_2)$ is gluable.  Now graph $H$ is obtained from the glueing of $H_1$ and $H_2$ along $\{y_1=y_2\}$ (denote the identified vertex $y$) in which $y$ is type-0 or
  type-1.  By Lemma~\ref{26}, $(H,\tau,\phi, y)$ is gluable where $\tau$ and $\phi$ are set as explained in the Lemma.

Now, assume that it represents directed cycle of length $2k$. 
Then depending on the cycle being of length two or higher we have the following two subcases. 

% Attaching a cycle and a stick
Case II.(c):
If $k=1$, then it represents a sail whose flag is 
  adjacent to the 3-vertex (of the sail) adjacent to the end of the sail.  
So $H$ is formed by a windmill? $H_1$ with axis $y_1$ and graph $H_2$ that 
  consists of a sail that ends in $y_2$ and its flag where $y_1$ and $y_2$ are identified. 
By induction, there is a set of types $\tau_1$ in which $y_1$ is not a 2-type and 
   a decent edge-labeling $\phi_1$ where $(H_1,\tau_1,\phi_1, y_1)$ is gluable. 
Now consider Example~\ref{19} that represents graph $H_2$ as shown in Figure~\ref{3}: 
  {\bf Figure 3: add x for the 2-vertex}
  $x$ is the 2-vertex, $w$ is the flag and $y$ is the end of the sail; i.e. the axis.
So, there is a set of types $\tau_2$ in which $y$ is not a 2-type and 
   a decent edge-labeling $\phi_2$ where $(H_2,\tau_2,\phi_2, y)$ is gluable. 
Now graph $H$ is obtained from the glueing of $H_1$ and $H_2$ along
  $\{y=y_2\}$ (denote the identified vertex by $y$) in which $y$ is type-0 or type-1. 
By Lemma~\ref{26}, $(H,\tau,\phi, y)$ is gluable where $\tau$ and $\phi$ are set as 
  explained in the Lemma. 


% Attaching a wheel
Case II.(d):
If $k\geq 2$, then it represents $k$ sails $S_1, S_2, \ldots, S_k$ and flags $f_1, f_2, \ldots, f_k$
   where each flag $f_i$ is adjacent to the 2-vertex of the sail $S_i$ and the 3-vertex next to the end of 
    the sail $S_{i+1}$. {\bf sums are taken in mod}
This represents a wheel in $H$. 
So $H$ is formed by a windmill? $H_1$ with axis $y_1$ and a wheel $W$ with axis $y_2$ 
   where $y_1$ and $y_2$ are identified. 
By induction, there is a set of types $\tau_1$ in which $y_1$ is not a 2-type and 
   a decent edge-labeling $\phi_1$ where $(H_1,\tau_1,\phi_1, y_1)$ is gluable. 
Recall that we assumed that $H$ contains no evil wheel.
So, $H_2$ is almost evil or not evil at all. 
Examples~\ref{21} and~\ref{22} represent both of these two cases (in Figures~\ref{5} and~\ref{6} $y$ is the axis of the wheel, i.e. $y_2$)
  and show that  there is a set of types $\tau_2$ in which $y_2$ is not a 2-type and 
   a decent edge-labeling $\phi_2$ where $(H_2,\tau_2,\phi_2, y_2)$ is gluable. 
Now graph $H$ is obtained from the glueing of $H_1$ and $H_2$ along
  $\{y_1=y_2\}$ (denote the identified vertex by $y$) in which $y$ is type-0 or type-1. 
By Lemma~\ref{26}, $(H,\tau,\phi, y)$ is gluable where $\tau$ and $\phi$ are set as 
  explained in the Lemma. 

Case III: 
If the strong component graph of the flag graph contains no isolated vertex, then the flag graph has a leaf. 
Based on the structure of the flag graph, there are two possibilities. 

Case III.(a):
The flag graph of $H$ has a leaf that is a sail vertex. 
Then the sail vertex has an edge that is directed toward a flag vertex which has an indegree at least two. 
$H$ is formed by a windmill $H_1$ with axis $y_1$ and a flag, say $w_1$,  and 
  a sail $H_2$ whose 2-vertex is adjacent to a flag say $w_2$ and ends in $y_2$ 
  where $y_1$ and $y_2$ are identified, as well as $w_1$ and $w_2$. 
By induction, there is a set of types $\tau_1$ in which $y_1$ is not a type-2 and 
   a decent edge-labeling $\phi_1$ where $(H_1,\tau_1,\phi_1, y_1)$ is gluable.  
Now, consider Example~\ref{17} that represents sail $H_2$ as follows: 
   $xv_1$ is the tip of the sail, 
   $w$ is the flag $w_2$ adjacent to the 2-vertex $x$, and $v_n$ is the axis, i.e. , $y_2$. 
So, there is a set of types $\tau_2$ in which $y_2$ is not a type-2 and 
   a decent edge-labeling $\phi_2$ where $(H_2,\tau_2,\phi_2, y_2)$ is gluable. 
Now graph $H$ is obtained from the glueing of $H_1$ and $H_2$ along
  $\{y_1=y_2, w_1 = w_2\}$ (denote the identified vertices $y$ and $f$, respectively) in which $y$ is type-0 or type-1. 
By Lemma~\ref{2-sum}, $(H,\tau,\phi, y)$ is gluable where $\tau$ and $\phi$ are set as 
  explained in the Lemma. 
{\bf it might be written so that it's the same case as Case II.(a). Case II.(a) requires 1-sum and Case III.(a) requires 2-sum.}

Case III.(b):
The flag graph of $H$ has a leaf that is a sail vertex. 
Then the sail vertex has an edge that is directed toward a flag vertex which has an indegree one. 
$H$ is formed by a windmill $H_1$ with axis $y_1$  and a graph shown in Figure~\ref{7}:
	graph $H_2$ contains a sail whose 2-vertex, say $x$ is adjacent to a flag say $w$ and ends in $y_2 = y$ 
Now, it can be seen that $H$ is obtained from $H_1$ and $H_2$ by identifying the two along the path $y, v_1, v_2$. 
Notice that the neighbour of flag $w$ in the other sail must be adjacent to the axis. 
By induction, there is a set of types $\tau_1$ in which $y_1$ is not a type-2 and 
   a decent edge-labeling $\phi_1$ where $(H_1,\tau_1,\phi_1, y_1)$ is gluable.  
{\bf add x and w to figure 7.}
Now, by Example~\ref{23-segments} that represents sail and the flag in $H_2$, 
   there is a set of types $\tau_2$ in which $y_2$ is not a type-2 and 
   a decent edge-labeling $\phi_2$ where $(H_2,\tau_2,\phi_2, y_2)$ is gluable. 
Now graph $H$ is obtained from the glueing of $H_1$ and $H_2$ along the path $y, v_1, v_2$
   (denote the identified vertices $y$ and $f$, respectively) in which $y$ is type-0 or type-1. 
By Lemma~\ref{32-pathsum}, $(H,\tau,\phi, y)$ is gluable where $\tau$ and $\phi$ are set as 
  explained in the Lemma. 

So far, we have considered all windmills using their flag graph representation. 
Now, to complete the proof, consider when a flag has a direct edge to the axis. 
The flag graph does not include such an edge as we explained earlier. 
Recall that an edge from a flag to the axis may only occure if the number of sails is one less than the degree of the axis. 

{\bf to be completed. depends on the notations we used earlier.}


\end{proof}

Lemma~\ref{?} and~\ref{?}  imply Theorem~\ref{thm:no-windmill}.



==> todo.tex <==
% todo.tex

\section*{TODO}
\begin{itemize}
%\item Figure 5 Last picture a +1 label must be -1
\item adding the scaling lemma (including infinity labels) Araujo
\item terminology of wheel elements?
\item text in figure 3 be removed
\item Figure 6 on the right requires correction: y is a type 1. text also needs to be updated
\item Add $x$ and $u$ label to Figure 3 (Fish)
\item Araujo $\leadsto$ Ara\'ujo
\item in gluing.tex, $y$ $\leadsto$ $y_1$,$y_2$
\item \dots
\item Delete TOC \& TODO
\end{itemize}
\begin{enumerate}[\S 1]
\item Intro: done 
\item Preliminaries: done
\item Windmills: done
\item Gluing: write some, read
\item no-windmill theorem 
\item discharging $\to$ Theorem~\ref{thm:main}
\item outlook
\end{enumerate}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "brock.tex"
%%% fill-column: 165
%%% End: 

